Enumeration Kernels of Polynomial Size for Cuts of Bounded Degree

Enumeration kernelization was first proposed by Creignou et al. [TOCS 2017] and was later refined by Golovach et al. [JCSS 2022] into two different variants: fully-polynomial enumeration kernelization and polynomial-delay enumeration kernelization. In this paper, we consider the d-CUT problem from the perspective of (polynomial-delay) enumeration kenrelization. Given an undirected graph G = (V, E), a cut F = (A, B) is a d-cut of G if every $u \in A$ has at most d neighbors in B and every $v \in B$ has at most d neighbors in A. Checking the existence of a d-cut in a graph is a well-known NP-hard problem and is well-studied in parameterized complexity [Algorithmica 2021, IWOCA 2021]. This problem also generalizes a well-studied problem MATCHING CUT (set d = 1) that has been a central problem in the literature of polynomial-delay enumeration kernelization. In this paper, we study three different enumeration variants of this problem, ENUM d-CUT, ENUM MIN-d-CUT and ENUM MAX-d-CUT that intends to enumerate all the d-cuts, all the minimal d-cuts and all the maximal d-cuts respectively. We consider various structural parameters of the input, e.g. vertex cover number, neighborhood diversity, and clique partition number. When vertex cover number and neighborhood diversity are considered as parameters, we provide polynomial-delay enumeration kernelizations of polynomial size for ENUM d-CUT and ENUM MAX-d-CUT and fully-polynomial enumeration kernels of polynomial size for ENUM MIN-d-CUT. When clique partition number is considered as the parameter, we provide bijective enumeration kernels for each of these three problems.

==> clique-partition-short-version-copy.tex <==
%nd-for-short-only

==> nd-short-version.tex <==
%nd-for-short-only

In this section, we give the proof sketches of the enumeration kernels when the parameters are {\bf (i)} neighborhood diversity, and {\bf (ii)} clique partition number.
Let $G$ be a graph and $\UU = \{X_1,\ldots,X_k\}$ be a neighborhood decomposition of $G$ with minimum number of modules.
If a module $X$ is a clique, then we call $X$ a {\em clique module}, and otherwise $X$ is an independent set and we call it an {\em independent module}.
A module is called {\em trivial} if it is independent module and not adjacent to any other module.
Finally, an independent module $X$ is {\em nice} if $|N_G(X)| \leq d$.
If a nice module $X$ has more than $3d+2$ vertices, then we say that $T = N_G(X)$ is a {\em bad} subsets.
Let $\YY$ denotes the collection of all such bad subsets.

{\ThmNDComb*}

\begin{proof}(Sketch)
The kernelization algorithms for each of the three problems are the same.
If the input graph $G$ has at most $(3d+2){\ndd}(G)$ vertices, then the kernelization algorithm outputs $H = G$ and we trivially have a bijective enumeration kernelization.
So, we assume that $G$ has more than $(3d+2){\ndd}(G)$ vertices.
If $X$ is an independent module and is not adjacent to any other module, then mark one vertex from $X$.
%For every other independent module $X$, mark $\min(3d+2, |X|)$ vertices of $X$.
If an independent module $X$ of $G$ is nice but has more than $3d+2$ vertices, then choose $d$ arbitrary marked vertices $u_1,\ldots,u_d$ and for every $i \in [d]$, attach a pendant clique $C_i$ with $2d+i+2$ vertices into $u_i$.
Replace the module $X$ by $(X \setminus \{u_i \mid i \in [d]\}$ and create new modules $\{u_i\}$ and $C_i \setminus \{u_i\}$.
If a module $X$ of $G$ does not satisfy any of the above properties, then mark $\min(2d+1, |X|)$ vertices from $X$.
Then output the graph $H$ with the modified neighborhood decomposition.
It is not hard to observe that ${\ndd}(H) \leq (2d+1){\nd}(G)$.

We describe the solution-lifting algorithm for {\enumdcut}.
Let $F' = (A', B')$ be a $d$-cut of $H$.
Observe that if a module $X$ of size at least $3d+3$ is nice, then $T = N_G(X)$ is a bad subset.
Moreover, $T \subseteq A'$ or $T \subseteq B'$ due to Lemma \ref{lem:neighborhood-break-up}.
If $T \subseteq A'$ and $F' \cap E(T, X') \neq \emptyset$, then the solution looks at $P' \subseteq X \cap B'$ with at most $\beta$ vertices.
If the sizes of these pendant cliques attached to $P'$ are $\{2d+2,\ldots,2d+\beta+1\}$, then the solution-lifting algorithm enumerates $P'$ and a collection of subsets of $X$ of size $\beta$ that contains at least one vertex not in $H$.
For every such subset $X' \subseteq X$, we replace $P'$ by $X'$ in $B'$.
Otherwise, the sizes of these attached pendant cliques are not $\{2d+2,\ldots,2d+\beta+1\}$ and we don't change the edge set
We repeat this process for every such bad subsets $T \in \YY$.
By arguments similar to Theorem \ref{thm:vc-result-main-1}, we can prove that this gives a polynomial-delay enumeration kernel for {\enumdcut} parameterized by the neighborhood diversity.
\end{proof}

